DADgraph: A Discourse-aware Dialogue Graph Neural Network for Multiparty Dialogue Machine Reading Comprehension

Multiparty Dialogue Machine Reading Comprehension (MRC) differs from traditional MRC as models must handle the complex dialogue discourse structure, previously unconsidered in traditional MRC. To fully exploit such discourse structure in multiparty dialogue, we present a discourse-aware dialogue graph neural network, DADgraph, which explicitly constructs the dialogue graph using discourse dependency links and discourse relations. To validate our model, we perform experiments on the Molweni corpus, a large-scale MRC dataset built over multiparty dialogue annotated with discourse structure. Experiments on Molweni show that our discourse-aware model achieves statistically significant improvements compared against strong neural network MRC baselines.

==> FriendsQA.tex <==

\begin{table}
    \begin{center}
    %\setlength{\tabcolsep}{10mm}{
        \begin{tabular}{l|l|c|c|c}
            \hline \bf   \bf   & \bf Train  & \bf Dev & \bf Test & \bf Total \\ 
            \hline
            Dialogues      & 977  &  122 & 123 & 1,222 \\
            %Utterances     & 79,487   &  7971 &  845 & 88,303\\ 
            %Relations     & 70,453    & 3,880 & 3,913 & 78,246  \\
            Questions     & 8,535 & 1,010 & 2,057 & 11,602  \\
            Answers     & 17,074   &  2,057 &  2,131 & 21,262\\ 
            \hline
        \end{tabular}%}
    \end{center}
    \caption{\label{font-table} The overview of FriendsQA for MRC.}
    \vspace{-0.16in}
\end{table}


==> case_dialogue1.tex <==
\begin{table}
    \begin{center}
        \setlength{\tabcolsep}{1mm}{
        \begin{tabular}{l}
          %  \hline \bf Dialogue 3  \\ 
            \hline
            \hline


\textit{sipher}: bacon5o there 's no `` fixmbr '' with \\
ubuntu . $U_1$ \\
\textit{morfic}: xaa is old acceleration architecture, exa \\
is the new one , font rendering is so much filepath  $U_2$\\
\textit{bacon5o}: i dont want ubuntu , it does n't \\
support my internet , thus i can not use it  $U_3$ \\
\textit{morfic}: your internet is different from mine ? \\
damn bush and his internets ! $U_4$\\
\textit{bacon5o}: my internet is differentwhy you ask ?  $U_5$\\
\textit{morfic}: your possesive `` my '' on the internet    $U_6$\\
\textit{bacon5o}: i use a wireless accesspoint that plugs into \\
my usb which then goes into my motherboard  $U_7$\\

        \hline
        \textbf{Q1}: What does \textit{Bacon5o} not want to use?  \\               
        \textbf{Gold answer}:ubuntu \\
        %\textbf{BERT answer}: likwidoxigen    \\
        \textbf{DialogueRNN}: a wireless accesspoint    \\
        \textbf{DialogueGCN}: it does n't support my internet    \\
        \textbf{Our model}: ubuntu    \\
        \hline
        \textbf{Q2}: Which one is new acceleration architecture? \\
        \textbf{Gold answer}: exa   \\
        %\textbf{BERT answer}: they worked excellently \\on dapper. \\
        \textbf{DialogueRNN}: xaa    \\
        \textbf{DialogueGCN}: xaa    \\
        \textbf{Our model}: exa    \\
        
        \hline
        \end{tabular}}
    \end{center}
    \caption{\label{font-table} An example from our Molweni test set with three speakers: \textit{sipher}, \textit{morfic}, and \textit{bacon5o}. Q1 and Q2 are two answerable questions, and we show gold answers and the output answers of DialogueRNN, DialogueGCN and our model.}
    %\vspace{-0.20in}
\end{table}


==> dialogue.tex <==

\begin{table}
    \begin{center}
        \setlength{\tabcolsep}{0.01mm}{
        \begin{tabular}{l}
           % \hline \bf Dialogue 1  \\ 
           \hline
            \hline
        
    1. \textbf{jimcooncat}:installing acroread gives me a 404 \\on maverick -- what to do ? \\
    2. \textbf{jrib}: where are you installing acroread from ?\\
    3. \textbf{elfranne}: people in the same local network ?  \\
    4. \textbf{llutz}: not network , on local computer \\
    5. \textbf{elfranne}: so its only available for `` localhost '' \\ and  not others on the same local network \\
    6. \textbf{jimcooncat}: thank you , i had forgot to update\\
    7. \textbf{llutz}: yes , `` other users on localhost ''  \\
        \hline
        
    \textbf{Q1}: Where does $llutz$ install acroread? \\ 
    \textbf{A1}: on local computer \\
    \textbf{Q2}: Why does $jimcoonact$ meet the 404 error? \\
    \textbf{A2}: forgot to update \\
    \textbf{Q3}: How did $erUSUL$ create a new partiton table?\\
    \textbf{A3}: NA.    \\
        \hline
        \end{tabular}}
    \end{center}
    \caption{\label{font-table} A dialogue from Molweni with its 3 questions, where Q1 and Q2 are answerable but Q3 is not.}
    %\vspace{-0.26in}
\end{table}


==> large.tex <==

\begin{table*}
\begin{center}
\begin{tabular}{c||l|l||l|c}
\hline
\multirow{2}{*}{\textbf{Method}}&
\multicolumn{2}{c||}{\textbf{FriendsQA}}& 
\multicolumn{2}{c}{\textbf{Molweni}} \\
\cline{2-5}
  & \textbf{EM} & \textbf{F1} & \textbf{EM} & \textbf{F1} \\
\hline
BERT-base & *** & *** & 45.3 & 58.0\\
BERT-large & *** & ***  & 51.8 & 65.5 \\
%BERT-wwm & 86.7 & 54.7 & 89.1 & 67.7 \\
%RoBERTa-base & --- & 52.0 & --- & 66.1 \\
%RoBERTa-large & 86.8 & 58.4 & 89.8 & 71.9\\
\hline
% GSN & & & & \\
DialogueRNN & *** & ***  & 49.4 & 64.6\\
DialogueGCN & *** & *** & 49.0 & 65.0\\
%\hline
DA DialogueGCN(auto) & *** & *** & 50.2 & 65.5 \\
DA DialogueGCN(gold) & --- & --- & 51.6 & 65.4\\
%Our-speaker & & & &  \\
\hline
Human performance & --- & --- & 64.3 & 80.2 \\
%Human-machine gap & 0 & 5.9 & -0.4 & 8.3 \\
\hline
\end{tabular}
\end{center}
\caption{\label{font-table} Results of machine reading comprehension for multiparty dialogues.}
%\vspace{-0.40in}
\end{table*}




==> mrc.tex <==
 
\section{Machine reading comprehension in multiparty dialogues}

In this section, we first define extractive machine reading comprehension for multiparty dialogues, then introduce the challenges of MRC for multiparty dialogue.\\

%Most of the existing machine reading comprehension tasks aim to understand a passage or passage and historical questions. There is little literature working on machine reading comprehension for dialogues \cite{chen2019reading,liu2019fast,sun2019dream}. DREAM is the first multiparty task machine reading comprehension dataset. However, more than 99\% dialogues in DREAM are two-party dialogues, and the proportion of multiparty dialogues is less than 1\%. Because two-party dialogues can be regarded as a special case of multiparty dialogues, we annotate more multiparty dialogues in our dataset to be helpful in the research of dialogues understanding. Besides, all questions in DREAM are the choice questions, but answers to our dataset are the span of input dialogue that would be more challenging.

%As we know, our dataset is the first corpus for multiparty dialogues reading comprehension. 
%Different from existing machine reading comprehension tasks, the input of this task is a multiparty dialogue, and we should answer some questions given the dialogue.  

\subsection{Task definition}
Given a multiparty dialogue $d$ and a question $q_i$, the task is a predict the answer $a_i$. There are two types of questions: answerable questions and unanswerable questions. If the question $q_i$ is answerable, the answer $a_i$ should be a continuous span in $d$. Otherwise, the answer $a_i$ should be $NA$.

\subsection{Challenges}

As mentioned above, the input is a multiparty dialogue. There are two key differences that thus distinguish this task from other MRC tasks:

\paragraph{C1. Utterances of multiparty dialogues are not coherent.} A passage is a continuous text where there is a discourse relation between every two adjacent sentences. Therefore, we can regard each paragraph in a passage as a linear discourse structure text. However, there could be no discourse relation between adjacent utterances in a multiparty dialogue. The discourse structure of a multiparty dialogue can be regarded as a dependency graph where each node is an utterance.

\paragraph{C2. Two-party dialogues can be regarded as the special case of multiparty dialogues.} The discourse structure of a multiparty dialogue is more complex than a two-party dialogue. In most cases, the discourse structure of a two-party dialogue is a dependency tree. Discourse relations in a two-party dialogue mostly happens among adjacent several utterances. However, two utterances may have discourse relations in a multiparty dialogue though they are very far. \\

An example of the discourse dependency graph of a multiparty dialogue is shown in Figure 1. In this example, there are six utterances in a multiparty dialogue, from utterance 1 to utterance 6. Especially, utterance 1 is the parent node of four utterances and utterance 6 has four parent nodes. We name this kind of discourse dependency structure as the radial structure which is the biggest difference with two-party dialogues. It would be essential to obtain the discourse structure of a multiparty dialogue for dialogue understanding. The discourse structure of dialogues would be introduced in detail in Section 3.

%\begin{figure}
%    \centering
%    \includegraphics[width=0.26\textwidth]{Figure/discourse_graph.pdf}
%    \caption{ A discourse dependency graph of a multiparty dialogues with six utterances. Each node represents an utterance, and the edge between two nodes represents discourse dependency relations. 
%    }
%    \label{fig:framework}
%\end{figure}



==> mrc_ablation.tex <==

\begin{table}
    \begin{center}
    %\setlength{\tabcolsep}{10mm}{
        \begin{tabular}{l|l|c}
            \hline \bf   \bf   & \bf EM  & \bf F1 \\ 
            \hline
            DADgraph      & 46.5   &  61.5 \\
            - w/o discourse relations     & 44.9   &  60.6 \\ 
            - w/o discourse structure      & 44.7   &  60.5 \\ 
            \hline
        \end{tabular}%}
    \end{center}
    \caption{\label{font-table} Results of ablation experiments on Molweni dataset.}
    \vspace{-0.16in}
\end{table}


==> mrc_overview.tex <==

\begin{table}
    \begin{center}
    %\setlength{\tabcolsep}{10mm}{
        \begin{tabular}{l|l|c|c|c}
            \hline \bf   \bf   & \bf Train  & \bf Dev & \bf Test & \bf Total \\ 
            \hline
            Dialogues      & 9,000   &  900 & 100 & 10,000 \\
            Utterances     & 79,487   &  7971 &  845 & 88,303\\ 
            %Relations     & 70,453    & 3,880 & 3,913 & 78,246  \\
            Questions     & 27,000 & 2,700 & 3,000 & 32,700  \\
            \hline
        \end{tabular}%}
    \end{center}
    \caption{\label{font-table} Overview of Molweni for MRC.}
    \vspace{-0.16in}
\end{table}


==> mrc_results.tex <==

\begin{table*}
\begin{center}
\begin{tabular}{c||l|l||l|c}
\hline
\multirow{2}{*}{\textbf{Method}}&
\multicolumn{2}{c||}{\textbf{EM}}& 
\multicolumn{2}{c}{\textbf{F1}} \\
\cline{2-5}
  & \textbf{Squad 2.0} & \textbf{Our} & \textbf{Squad 2.0} & \textbf{Our} \\
\hline
BiDAF-No-Answer (BNA) & 59.2 & *** & 62.1 & ***\\
AOA & --- & *** & --- & ***\\
\hline
%DocQA & 59.3 & *** & 62.3 & *** \\
%DocQA + ELMo & 63.4 & *** & 66.3 & *** \\
%BiDAF-ensemble & 73.3 & *** & 81.1 & *** \\
BERT-base & 73.1 & 45.3 & 76.2 & 58.0\\
BERT-large & 80.0 & 51.8 & 83.1 & 65.5 \\
BERT-wwm & 86.7 & 54.7 & 89.1 & 67.7 \\
RoBERTa-base & --- & 52.0 & --- & 66.1 \\
RoBERTa-large & 86.8 & 58.4 & 89.8 & 71.9\\
\hline
% GSN & & & & \\
DialogueRNN & --- &  45.9 & --- & 60.4\\
DialogueGCN & ---& 44.7 & --- & 60.5\\
%\hline
DA DialogueGCN(auto) & --- & 45.4 & --- & 60.8 \\
DA DialogueGCN(gold) & --- & 46.5 & --- & 61.5\\
%Our-speaker & & & &  \\
\hline
Human performance & 86.8 & 64.3 & 89.4 & 80.2 \\
%Human-machine gap & 0 & 5.9 & -0.4 & 8.3 \\
\hline
\end{tabular}
\end{center}
\caption{\label{font-table} Results of machine reading comprehension for multiparty dialogues.}
%\vspace{-0.40in}
\end{table*}


==> mrc_results_molweni.tex <==
\begin{table}
    \begin{center}
    %\setlength{\tabcolsep}{10mm}{
        \begin{tabular}{l|l|c}
            \hline \bf   \bf   & \bf EM  & \bf F1 \\
            \hline
BiDAF \cite{seo2016BiDAF} & 22.9 & 39.8\\
DocQA \cite{clark2018simple}& 42.5 & 56.0\\
%\hline
BERT \cite{devlin2019bert}  & 45.3 & 58.0\\
DialogueRNN \cite{majumder2019dialoguernn} & 45.4 & 60.9\\
DialogueGCN \cite{ghosal2019dialoguegcn}  & 45.7 & 61.0\\
%\hline
%DA DialogueGCN(auto)  & 45.4 & 60.8 \\
\hline
DADgraph (Our)  & \textbf{46.5} & \textbf{61.5}\\
\hline
Human performance  & 64.3 & 80.2 \\
\hline
\end{tabular}%}
\end{center}
\caption{\label{font-table} Results on Molweni dataset.}
    %\vspace{-0.16in}
\end{table}


==> results_friends.tex <==

\begin{table}
    \begin{center}
    %\setlength{\tabcolsep}{10mm}{
        \begin{tabular}{l|l|c}
            \hline \bf   \bf   & \bf EM  & \bf F1 \\
            \hline
        BiDAF \cite{seo2016BiDAF} & 11.1 & 21.5 \\
        DocQA \cite{clark2018simple} & 30.1 & 43.4 \\
%\hline
    BERT \cite{devlin2019bert}&  48.3 & 63.6 \\
    DialogueRNN \cite{majumder2019dialoguernn} & *** & ***  \\
    DialogueGCN \cite{ghosal2019dialoguegcn}& *** & *** \\
%\hline
\hline
    DADgraph* & *** & ***  \\
            \hline
        \end{tabular}%}
    \end{center}
    \caption{\label{font-table} Results on the FriendsQA dataset. DA-DialogueGCN* method adopts the discourse structure from discourse parser.}
    \vspace{-0.16in}
\end{table}


==> running_example.tex <==

\begin{table}
    \begin{center}
        \setlength{\tabcolsep}{0.01mm}{
        \begin{tabular}{l}
            \hline \bf Dialogue 1  \\ 
            \hline
            \hline
        
    1. \textbf{frankfurter}: maco where do i find the path \\ to the file ? \\
    2. \textbf{actionparsnip}: you can use lynx to web browse \\ to the file \\
    3. \textbf{maco}: im confused now . isnt that just full of  isos ?  \\
    4. \textbf{actionparsnip}: read the 2nd link : url \\
    5. \textbf{maco}: oh sorry i thought you were responding to \\ the tarball thing \\
    6. \textbf{red2kic}: well , only if the hard drive failed . \\
    7. \textbf{maco}: using a separate partition is no guarantee \\ against a disk failure .  \\
    8. \textbf{maco}: right , which is why i thought people \\ usually had backups . \\
        \hline
        
    \textbf{Q1}: How can FrankFurter find the path to \\ the file?   \\                     
    \textbf{A1}: use lynx to web browse to the file \\
    \textbf{Q2}: Why does Maco think people usually \\ had backups? \\
    \textbf{A2}: using a separate partition is no guarantee \\ against  a disk failure \\
    \textbf{Q3}: What is Red2kic's advice? \\
    \textbf{A3}: NA.    \\
        

        \hline
        \end{tabular}}
    \end{center}
    \caption{\label{font-table} A dialogue from Molweni with its 3 questions, where Q1 and Q2 are answerable but Q3 is not.}
    \vspace{-0.26in}
\end{table}


==> two_overview.tex <==

\begin{table*}
\begin{center}
\begin{tabular}{c||c|c|c||c|c|c}
\hline
\multirow{2}{*}{\textbf{Method}}&
\multicolumn{3}{c||}{\textbf{Molweni}}& 
\multicolumn{3}{c}{\textbf{FriendsQA}} \\
\cline{2-7}
  & \textbf{Train} & \textbf{Dev} & \textbf{Test}  & \textbf{Train} & \textbf{Dev} & \textbf{Test} \\
\hline
%BiDAF-No-Answer (BNA) & 59.2 & *** & 62.1 & ***\\
%DocQA & 59.3 & *** & 62.3 & *** \\
%DocQA + ELMo & 63.4 & *** & 66.3 & *** \\
%BiDAF-ensemble & 73.3 & *** & 81.1 & *** \\
Dialogues & 9,000 & 900 & 100 & 973 & 113 & 136\\
Utterances & 79,487 & 7,971 & 845 & 21,607 & 2,336 & 2,847\\
Questions & 27,000 & 2,700 & 3,000 & 19,630 & 1,201 & 1,182\\
%RoBERTa-base & --- & 52.0 & --- & 66.1 \\
%RoBERTa-large & 86.8 & 58.4 & 89.8 & 71.9\\

\hline
\end{tabular}
\end{center}
\caption{\label{font-table} The overview of Molweni dataset and FriendsQA dataset.}
\vspace{-0.10in}
\end{table*}

